Power Side Channels in Security ICs: Hardware Countermeasures

Power side-channel attacks are a very effective cryptanalysis technique that can infer secret keys of security ICs by monitoring the power consumption. Since the emergence of practical attacks in the late 90s, they have been a major threat to many cryptographic-equipped devices including smart cards, encrypted FPGA designs, and mobile phones. Designers and manufacturers of cryptographic devices have in response developed various countermeasures for protection. Attacking methods have also evolved to counteract resistant implementations. This paper reviews foundational power analysis attack techniques and examines a variety of hardware design mitigations. The aim is to highlight exposed vulnerabilities in hardware-based countermeasures for future more secure implementations.

==> figures/nand2.tex <==
\scalebox{1} % Change this value to rescale the drawing.
{
  \begin{pspicture}(0,-2.8552785)(3.7996485,2.9)
  \psline[linewidth=0.04cm](1.4841797,2.24)(1.8041797,2.24)
  \psline[linewidth=0.04](1.6441798,2.24)(1.6441798,1.76)(1.3241796,1.76)(1.3241796,1.12)(1.6441798,1.12)(1.6441798,0.64)(2.2841797,0.64)(2.2841797,-0.32)(1.9641796,-0.32)(1.9641796,-0.96)(2.2841797,-0.96)(2.2841797,-1.44)(1.9641796,-1.44)(1.9641796,-2.08)(2.2841797,-2.08)(2.2841797,-2.56)
  \psline[linewidth=0.04](2.2841797,0.64)(2.9241798,0.64)(2.9241798,1.12)(2.6041799,1.12)(2.6041799,1.76)(2.9241798,1.76)(2.9241798,2.24)
  \psline[linewidth=0.04cm](2.7641797,2.24)(3.0841799,2.24)
  \psline[linewidth=0.04cm](1.1641797,1.76)(1.1641797,1.12)
  \psline[linewidth=0.04cm](2.4441798,1.76)(2.4441798,1.12)
  \psline[linewidth=0.04cm](1.8041797,-0.32)(1.8041797,-0.96)
  \psline[linewidth=0.04cm](1.8041797,-1.44)(1.8041797,-2.08)
  \rput{-180.0}(4.56836,-5.44){\pstriangle[linewidth=0.04,dimen=outer](2.28418,-2.88)(0.32,0.32)}
  \usefont{T1}{pcr}{m}{n}
  \rput(0.07488281,-1.495){B}
  \usefont{T1}{pcr}{m}{n}
  \rput(0.13535157,1.705){A}
  \psline[linewidth=0.04](0.84417975,1.44)(0.84417975,-0.64)(1.8041797,-0.64)
  \psline[linewidth=0.04cm,dotsize=0.07055555cm 2.0]{-oo}(2.1241798,1.44)(2.4441798,1.44)
  \psline[linewidth=0.04cm,dotsize=0.07055555cm 2.0]{-oo}(0.044179693,1.44)(1.1641797,1.44)
  \psline[linewidth=0.04](2.1241798,1.44)(2.1241798,2.88)(0.5241797,2.88)(0.5241797,-1.76)(1.8041797,-1.76)
  \psline[linewidth=0.04cm](0.5241797,-1.76)(0.044179693,-1.76)
  \psdots[dotsize=0.12](0.5241797,-1.76)
  \psdots[dotsize=0.12](0.84417975,1.44)
  \usefont{T1}{pcr}{m}{n}
  \rput(2.7630959,2.485){\scriptsize $V_{dd}$}
  \usefont{T1}{pcr}{m}{n}
  \rput(1.4830958,2.485){\scriptsize $V_{dd}$}
  \usefont{T1}{pcr}{m}{n}
  \rput(2.290546,-0.6878353){\scriptsize N1}
  \usefont{T1}{pcr}{m}{n}
  \rput(2.290546,-1.7596855){\scriptsize N2}
  \usefont{T1}{pcr}{m}{n}
  \rput(1.7067704,1.4614192){\scriptsize P1}
  \usefont{T1}{pcr}{m}{n}
  \rput(2.9615715,1.4614192){\scriptsize P2}
  \psdots[dotsize=0.12](2.2996485,0.62)
  \psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.2996485,0.1)(3.7796485,0.1)
  \usefont{T1}{pcr}{m}{n}
  \rput(3.220244,-0.075){\scriptsize Output}
  \psdots[dotsize=0.12](2.2798243,0.1)
  \end{pspicture}
}

